PQC Migration: End-to-End Performance Profiling of Post Quantum Cryptographic Algorithms in mTLS

Emerging quantum computers threaten to break the classical key exchange algorithms. To safeguard against these threats, migration to new quantum-safe algorithms is underway and expected to be expedited. Though resistant to attacks, the quantum safe algorithms may impact the real-world performance due to their large key lengths. In this work, we analyze the end-to-end performance of the Transport Layer Security (TLS) protocol with the post-quantum (PQ) and hybrid cryptographic algorithms standardized by NIST. We develop a test setup to evaluate the performance of TLS connections between a client and a server under various network conditions. We focus on the impact of the new algorithms on the speed (throughput, connection time) and sustainability (energy, CPU cycles) of TLS 1.3. Our analysis demonstrates that the standardized post-quantum algorithms do not introduce any measurable performance degradations in TLS 1.3, despite their larger key lengths. However, hybrid algorithms introduce noticeable performance degradation, which becomes increasingly pronounced under adverse network conditions. Our analysis suggests that migration to hybrid algorithms should be ``network condition aware'' as poor network conditions can severely degrade performance in TLS 1.3. We provide anonymised link to the code and a web interface to analyse performance of various combination of algorithms.

==> bib.tex <==
Stebila, D., Mosca, M. (2017). Post-quantum Key Exchange for the Internet and the Open Quantum Safe Project. In: Avanzi, R., Heys, H. (eds) Selected Areas in Cryptography – SAC 2016. SAC 2016. Lecture Notes in Computer Science(), vol 10532. Springer, Cham. https://doi.org/10.1007/978-3-319-69453-5_2
